Detecting Sybil Attacks using Proofs of Work and Location in VANETs

In this paper, we propose a Sybil attack detection scheme using proofs of work and location. The idea is that each road side unit (RSU) issues a signed time-stamped tag as a proof for the vehicle's anonymous location. Proofs sent from multiple consecutive RSUs is used to create vehicle trajectory which is used as vehicle anonymous identity. Also, one RSU is not able to issue trajectories for vehicles, rather the contributions of several RSUs are needed. By this way, attackers need to compromise an infeasible number of RSUs to create fake trajectories. Moreover, upon receiving the proof of location from an RSU, the vehicle should solve a computational puzzle by running proof of work (PoW) algorithm. So, it should provide a valid solution (proof of work) to the next RSU before it can obtain a proof of location. Using the PoW can prevent the vehicles from creating multiple trajectories in case of low-dense RSUs. Then, during any reported event, e.g., road congestion, the event manager uses a matching technique to identify the trajectories sent from Sybil vehicles. The scheme depends on the fact that the Sybil trajectories are bounded physically to one vehicle; therefore, their trajectories should overlap. Extensive experiments and simulations demonstrate that our scheme achieves high detection rate to Sybil attacks with low false negative and acceptable communication and computation overhead.

==> Figures/PoW Experiment/PoW_experiment.tex <==
\section{Experimental Analysis of Trajectory Generation with PoW Support}
\label{sec:ExperimentalAnalysisofTrajectoryGenerationwithPoWSupport}

\subsection{Overview}
\label{sec:Overview}

A promising approach to eliminate Sybil attack in VANET is the timestamp-based technique as proposed in Footprint \cite{RefWorks:doc:5b4d0f84e4b06133484c6f48}. In this technique, each vehicle authenticates itself using a unique sequence of authorized timestamps issued by RSUs. This sequence of timestamps is called a trajectory. A main property of this technique is that it provides anonymity for vehicles. A major drawback is that vehicles are able to generate arbitrarily many trajectories simultaneously, which faces two problems. First, more trajectories incur additional overhead to RSUs as well as to the verifier of trajectories, and second, a large number of trajectories can increase the chance for an attacker to succeed launching Sybil attack, even after applying an elimination method. 

\subsection{Objective}
\label{sec:Objective}

This experiment faces the aforementioned problems, and therefore the objective of this experiment is to limit the number of trajectories each vehicle can generate by utilizing the concept of PoW. The general approach works as follows. Each timestamp issued by an RSU can be used to derive a unique seed value for a PoW algorithm. While a vehicle approaches an RSU, it runs the PoW algorithm using the seed value it has derived from the most recent timestamp it obtained. Once the vehicle arrives at the RSU, it submits the best PoW result to the RSU, where the best PoW result is defined as the hash output with the lowest value. The longer it takes a vehicle to travel between two RSUs, the more time it has available to generate a PoW and hence the lower the best PoW result should become. Due to the limitation of a vehicle’s computational resources, it would be difficult for a vehicle to generate multiple trajectories simultaneously, because it would have to generate a separate PoW for each trajectory. Calculating multiple PoWs simultaneously will sacrifice difficulty level of obtained PoW results. Upon arrival of the vehicle at an RSU, the RSU can evaluate whether the obtained PoW result corresponds to the expected difficulty based on the vehicle’s travel time. If the result of a PoW does not meet the required difficulty, an RSU can refuse contributing a timestamp to the corresponding trajectory, forcing the vehicle to start over with a new trajectory.

\subsection{Implementation}
\label{sec:Implementation}

Our experiment proves feasibility of this approach and it shows that this method can limit the number of simultaneously generated trajectories by a single vehicle. 

The PoW algorithm used in our experiment is the Hashcash algorithm as used in the Bitcoin cryptocurrency. This experiment is based on the following assumptions:

\begin{itemize}
	\item Computational power: All vehicles have the same computational power and each vehicle uses the same constant hash rate.
	\item Vehicles' velocity: All vehicles are moving with constant velocity and do not stop at any time.
	\item RSU distribution: All RSUs are equally distributed, meaning that the distance between any two neighboring RSUs is the same.
	\item Travel time between RSUs: Based on the two previous assumptions, the time it takes any vehicle to travel between two RSUs is constant.
\end{itemize}

The first step of our experiment shows a technique that allows RSUs to determine the threshold a vehicle’s PoW result should fall below after a certain time $t$. In the remainder of this chapter we will refer to this threshold as target. In this step of the experiment we ran the PoW algorithm for $n$ times and plotted the probabilities of obtaining PoW results within a range for different times, respectively. The results for $n=1000$ and $t=10, 30, 90$ and $130 sec.$, respectively are shown in Fig. \ref{fig:dmf_target_10_30_90_130} and \ref{fig:cdf_target_10_30_90_130}.

\begin{figure}[tbp]
	\setlength{\abovecaptionskip}{0.3cm}   % 0.5cm as an example
	\setlength{\belowcaptionskip}{0.0cm}   % 0.5cm as an example
	\centering
	\includegraphics[scale=0.4]{\jobname-content/figures/dmf_target_10_30_90_130.png}
	\caption{Probability mass functions of PoW results with constant times.}
	\vspace{0mm}
	\label{fig:dmf_target_10_30_90_130}
\end{figure}

\begin{figure}[tbp]
	\setlength{\abovecaptionskip}{0.3cm}   % 0.5cm as an example
	\setlength{\belowcaptionskip}{0.0cm}   % 0.5cm as an example
	\centering
	\includegraphics[scale=0.4]{\jobname-content/figures/cdf_target_10_30_90_130.png}
	\caption{Cumulative distribution functions of PoW results with constant times.}
	\vspace{0mm}
	\label{fig:cdf_target_10_30_90_130}
\end{figure}

Based on the obtained results shown in Fig. \ref{fig:pmf_target_10_30_90_130} and Fig. \ref{fig:cdf_target_10_30_90_130}, the expected targets with given probabilities and after certain times can be derived. This is shown in Fig. \ref{fig:target_over_time_succ_rate_95_90_85_80}. Given Fig. \ref{fig:target_over_time_succ_rate_95_90_85_80}, an RSU is able to determine the target it should expect from a vehicle’s PoW result.

\begin{figure}[tbp]
	\setlength{\abovecaptionskip}{0.3cm}   % 0.5cm as an example
	\setlength{\belowcaptionskip}{0.0cm}   % 0.5cm as an example
	\centering
	\includegraphics[scale=0.4]{\jobname-content/figures/target_over_time_succ_rate_95_90_85_80.png}
	\caption{ }
	\vspace{0mm}
	\label{fig:target_over_time_succ_rate_95_90_85_80}
\end{figure}

The second step determines the probabilities of success for honest and malicious vehicles, respectively, considering an increasing trajectory length and a number of varying targets obtained from step one. 

For this step we sequentially created PoWs below a certain target and counted how many of these PoWs were found within time $t$. Based on the obtained results, the following two cases can be observed:

\begin{itemize}
	\item Success of honest vehicles. An honest vehicles is generating a successful trajectory, if it generates a PoW result below the required target for any RSU it approaches. Therefore, if at least one PoW result below the target was obtained within the relevant time, an honest vehicle succeeds.
	\item Success of malicious vehicles. A malicious vehicle is generating successful trajectories, if it generates multiple PoW results below the required target for any RSU it approaches. In this experiment the number of solved PoWs per time represents the number of timestamps a vehicle was able to maintain while travelling between two RSUs.
\end{itemize}

Concatenating the counts for consecutive instances of time $t$, we are able to represent trajectories with lengths higher than one. However, in the case of malicious vehicles, only the lowest count of solved PoWs in a trajectory sequence was considered the actual number of successfully generated trajectories. 

This count represents the number of timestamps a vehicle was able to maintain while travelling between two RSUs. Concatenating the counts for consecutive instances of time $t$, we were able to represent trajectories with lengths higher than one. However, only the lowest count of solved PoWs in a trajectory sequence was considered the actual number of successfully generated trajectories. 

Given a constant target, we generated a set of $n=1000$ samples for every increment of trajectory length, respectively. Then, we plotted the probability of successfully generating trajectories for each set, respectively. Finally, we repeated the aforementioned procedure with different targets. The results are shown in Fig. \ref{fig:honest_success_probability} and Fig. \ref{fig:malicious_success_probability_98}.

\begin{figure}[tbp]
	\setlength{\abovecaptionskip}{0.3cm}   % 0.5cm as an example
	\setlength{\belowcaptionskip}{0.0cm}   % 0.5cm as an example
	\centering
	\includegraphics[scale=0.4]{\jobname-content/figures/honest_success_probability.png}
	\caption{Probability of success for honest vehicles in generating trajectories with increasing length.}
	\vspace{0mm}
	\label{fig:honest_success_probability}
\end{figure}

\begin{figure}[tbp]
	\setlength{\abovecaptionskip}{0.3cm}   % 0.5cm as an example
	\setlength{\belowcaptionskip}{0.0cm}   % 0.5cm as an example
	\centering
	\includegraphics[scale=0.4]{\jobname-content/figures/malicious_success_probability_98.png}
	\caption{Probability of success for malicious vehicles in generating multiple trajectories with increasing lengths.}
	\vspace{0mm}
	\label{fig:malicious_success_probability_98}
\end{figure}

\subsection{Conclusion}
\label{sec:Conclusion}

From Fig. \ref{fig:honest_success_probability} and Fig. \ref{fig:malicious_success_probability_98} can be seen that by slightly sacrificing the success rate for honest vehicles to generate a valid trajectory, we can limit the ability of malicious vehicles to maintain multiple trajectories simultaneously and hence reduce the success rate in launching Sybil attack. The higher the length of trajectories, the lower the success of generating multiple trajectories at the same time. Increasing the difficulty level of the PoW (lower target) reduces the number of simultaneously generated trajectories. However, setting the target too low can result in honest vehicles not being able to obtain a single trajectory, which incurs in false positives. 
